Revisiting Deep Subspace Alignment for Unsupervised Domain Adaptation

Unsupervised domain adaptation (UDA) aims to transfer and adapt knowledge from a labeled source domain to an unlabeled target domain. Traditionally, subspace-based methods form an important class of solutions to this problem. Despite their mathematical elegance and tractability, these methods are often found to be ineffective at producing domain-invariant features with complex, real-world datasets. Motivated by the recent advances in representation learning with deep networks, this paper revisits the use of subspace alignment for UDA and proposes a novel adaptation algorithm that consistently leads to improved generalization. In contrast to existing adversarial training-based DA methods, our approach isolates feature learning and distribution alignment steps, and utilizes a primary-auxiliary optimization strategy to effectively balance the objectives of domain invariance and model fidelity. While providing a significant reduction in target data and computational requirements, our subspace-based DA performs competitively and sometimes even outperforms state-of-the-art approaches on several standard UDA benchmarks. Furthermore, subspace alignment leads to intrinsically well-regularized models that demonstrate strong generalization even in the challenging partial DA setting. Finally, the design of our UDA framework inherently supports progressive adaptation to new target domains at test-time, without requiring retraining of the model from scratch. In summary, powered by powerful feature learners and an effective optimization strategy, we establish subspace-based DA as a highly effective approach for visual recognition.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> algo_progressive_DA.tex <==
\RestyleAlgo{boxruled}
\begin{algorithm}[t]

\caption{Proposed algorithm for unsupervised progressive domain adaptation}
	\label{algo:algo}
	\KwIn{
	TAFE trained from source $\rightarrow$ target_1
	Labeled source features $\{\mathrm{Z}_s,\mathrm{y}_s\} $ and 
	target_1 features $\{\mathrm{Z}_{t1}\}$ and target_2 features from TAFE $\mathcal{F}_{\Omega}$.
	Source and target subspaces $\mathrm{W}_s$, $\mathrm{W}_t$ }
	
	\textbf{Initialize}: $\mathcal{G}_{\Psi}$ from $\mathcal{F}_{\Omega}$, $\Phi$ using \eqref{eq:globalsoln}; Hyper-parameters $\gamma_c,\gamma_{cb}, n_{iter},T_1,T_2 $.

\textbf{Training Phase}:\newline  
     Split: $\mathrm{Z}_S^{\dagger} , \mathrm{Z}_S^{\ddagger} \leftarrow  \mathrm{Z}_S$ and $\mathrm{Z}_T^{\dagger} , \mathrm{Z}_T^{\ddagger} \leftarrow \mathrm{Z}_T$ \newline  
 	\For{iter \textbf{in} $n_{iter}$}{
 	     \tcp{ update $\mathcal{G}_{\Psi}$}
 	    \For{$t_1$ \textbf{in} $T_1$}{
           		   
			Compute $\bm\hat{\mathrm{Z}}_t^{\dagger} = \mathrm{Z}_t^{\dagger}\mathrm{W}_t\mathrm{\Phi}^*\mathrm{W}_s^T $ following \eqref{eq:reproj}\;
			$\bm\hat{\mathrm{y}}_s^{\dagger} = \mathcal{G}_{\Psi}(\bm\hat{\mathrm{Z}}_s^{\dagger})$\; 
			$\bm\hat{\mathrm{y}}_t^{\dagger} = \mathcal{G}_{\Psi}(\bm\hat{\mathrm{Z}}_t^{\dagger})$\;
			
			
			Compute $\mathrm{L}_{\mathcal{G}}$ using \eqref{eqn:classifier_loss}\;
		
			Update $\Psi^* = \arg \min_{\Psi} \mathrm{L}_{\mathcal{G}} $ \;}
            
	        \tcp{ update $\mathcal{A}_{\Phi}$}
			\For{$t_2$ \textbf{in} $T_2$}{
		
			
			Compute $\bm\hat{\mathrm{Z}}_t^{\ddagger} $ using \eqref{eq:reproj}\; 
			Compute $\bm\hat{\mathrm{y}}_t^{\ddagger} =\mathcal{G}_{\Psi^*}(\bm\hat{\mathrm{Z}}_t^{\ddagger})  $; 

			Compute $\mathcal{L}_{\mathcal{A}}$ using \eqref{eqn:loss_A}\; 
			Update $\mathrm{\Phi}^* = \arg \min_{\Phi} \mathrm{L}_{\mathcal{A}_{\Phi}} $ \;
			}
 		}


\end{algorithm}


==> tables/pda_office31.tex <==
\begin{table*}[h]
    \addtolength{\tabcolsep}{6pt}
    \centering 
        \renewcommand{\arraystretch}{1.4}
    
    \resizebox{0.75\textwidth}{!}{%
    \begin{tabular}{c|cccccc|c}
    	\hline
        \textbf{Method}
        & \textbf{A} $\rightarrow$ \textbf{W} & \textbf{D} $\rightarrow$ \textbf{W} &\textbf{W} $\rightarrow$ \textbf{D} & \textbf{A} $\rightarrow$ \textbf{D} & \textbf{D} $\rightarrow$ \textbf{A} & \textbf{W} $\rightarrow$ \textbf{A} & \textbf{Avg} \\
        \hline
        % ResNet~\cite{ResNet} & 54.52 & 94.57 & 94.27 & 65.61 & 73.17 & 71.71 & 75.64\\
        DAN~\cite{DAN} & 46.44 & 53.56 & 58.60 & 42.68 & 65.66 & 65.34 & 55.38 \\
        DANN~\cite{cite:JMLR16RevGrad} & 41.35 & 46.78 & 38.85 & 41.36 & 41.34 & 44.68 & 42.39  \\
        ADDA~\cite{cite:CVPR17ADDA} & 43.65 & 46.48 & 40.12 & 43.66 & 42.76 & 45.95 & 43.77 \\
        RTN~\cite{cite:NIPS16RTN} & 75.25 & \textbf{97.12} & \textbf{98.32} & 66.88 & \textbf{85.59} & \textbf{85.70} & \textbf{84.81} \\
        JAN~\cite{cite:ICML17JAN} & 43.39 & 53.56 & 41.40 & 35.67 & 51.04 & 51.57 & 46.11 \\
        LEL~\cite{LEL} & \textit{\textbf{73.22}} & \textit{\textbf{93.90}} & 96.82 & \textit{\textbf{76.43}} & \textit{\textbf{83.62}} & \textit{\textbf{84.76}} & \textit{\textbf{84.79}} \\
        \textbf{Ours} & \textbf{81.69} & 93.8 & \textit{\textbf{98.03}} & \textbf{85.9} & 76.2 & 83.4 & 83.01\\
        \hline
        \rowcolor{gray!25} PADA & {86.54} & {99.32} & {100} & 82.17 & {92.69} & {95.41} & {92.69} \\ 
        
    	\hline
    \end{tabular}%
    }
    \caption{Accuracy of partial domain adaptation tasks on \emph{Office-31} (ResNet-50)}
    \label{tab:pda_office31}
\end{table*}


==> tables/visda.tex <==
\begin{table}[t]
    %\large
    \begin{center}
    \renewcommand{\arraystretch}{1.4}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ccccccccccccccc}
        \hline
        Method&plane& bcycl&	bus&	car&	horse&	knife&	mcycl&	person&	plant&	sktbd&	train&	truck & Mean & Overall Acc   \\\hline
        No Adaptation & 79.56 & 12.51& 74.32& 83.04 & 75.97 & 2.79 & 85.23 & 14.63 & 68.47 & 19.2& 72.56 &5.803& 49.51 & 54.2\\
   
        
        JAN\cite{JAN} & - & -& -& -& -& -& -& -& -& -& -&  - & -& 61.6 \\

        
       JAN\cite{JAN} & - & -& -& -& -& -& -& -& -& -& -&  - & -& 61.6 \\
 
        
        CDAN\cite{CDAN} & - & -& -& -& -& -& -& -& -& -& -&  - & -& 70.2\\
     
       Ours & 96.7 & 86.7& 79.01 &48.9 & 93.6 & 91.1 & 82.2 & 74.1 & 89.1 & 79.2& 88.9 & 52.1&79.9& \textbf{76.3}\\
        
        
        \hline
        \end{tabular}}
  

    
    \end{center}
    \caption{\small{Classification accuracy on VISDA  dataset}}
    \label{table:visda}
    \end{table}

